O1-Pruner: Length-Harmonizing Fine-Tuning for O1-Like Reasoning Pruning

Recently, long-thought reasoning LLMs, such as OpenAI's O1, adopt extended reasoning processes similar to how humans ponder over complex problems. This reasoning paradigm significantly enhances the model's problem-solving abilities and has achieved promising results. However, long-thought reasoning process leads to a substantial increase in inference time. A pressing challenge is reducing the inference overhead of long-thought LLMs while ensuring accuracy. In this paper, we experimentally demonstrate that long-thought reasoning models struggle to effectively allocate token budgets based on problem difficulty and reasoning redundancies. To address this, we propose Length-Harmonizing Fine-Tuning (O1-Pruner), aiming at minimizing reasoning overhead while maintaining accuracy. This effective fine-tuning method first estimates the LLM's baseline performance through pre-sampling and then uses RL-style fine-tuning to encourage the model to generate shorter reasoning processes under accuracy constraints. This allows the model to achieve efficient reasoning with lower redundancy while maintaining accuracy. Experiments on various mathematical reasoning benchmarks show that O1-Pruner not only significantly reduces inference overhead but also achieves higher accuracy, providing a novel and promising solution to this challenge. Our code is coming soon at https://github.com/StarDewXXX/O1-Pruner

==> text/impact.tex <==
\section{Impact Statement}
This paper presents work aimed at addressing a critical challenge in the domain of long-thought reasoning Large Language Models (LLMs): balancing inference efficiency with accuracy. By proposing Length-Harmonizing Fine-Tuning (\method{}), we offer a novel approach to optimize reasoning processes by reducing redundancies and aligning token budgets with problem difficulty. Our work highlights the transformative potential of \method{} in enhancing the reasoning efficiency of LLMs without sacrificing performance. Experimental results on mathematical reasoning benchmarks demonstrate that \method{} significantly reduces inference overhead while improving accuracy, paving the way for more practical and scalable LLM applications across diverse domains. This advancement underscores the importance of innovative fine-tuning methods in overcoming fundamental limitations of long-thought reasoning paradigms, contributing to the broader evolution of LLM capabilities in both academic and practical contexts.
